s-process Enriched Evolved Binaries in the Galaxy and the Magellanic Clouds

Post-asymptotic giant branch stars (post-AGB) in binary systems, with typical orbital periods between ~100 to ~1000 days, result from a poorly understood interaction that terminates their precursory AGB phase. The majority of these binaries display a photospheric anomaly called 'chemical depletion', thought to arise from an interaction between the circumbinary disc and the post-AGB star, leading to the reaccretion of pure gas onto the star, devoid of refractory elements due to dust formation. In this paper, we focus on a subset of chemically peculiar binary post-AGBs in the Galaxy and the Magellanic Clouds (MCs) whose high-resolution optical spectroscopic study revealed a carbon and s-process enrichment, contrary to the commonly observed photospheric chemical depletion. Using spectral energy distribution (SED) fitting and period-luminosity-colour (PLC) relation methods, we determine the luminosity of the targets ($2700-8300L_{\odot}$), which enables confirmation of their evolutionary phase and estimation of initial masses (as a function of metallicity) ($1-2.5M_{\odot}$). In conjunction with predictions from dedicated ATON stellar evolutionary models, our results indicate a predominant intrinsic enrichment of carbon and s-process elements in our binary post-AGB targets. We qualitatively rule out extrinsic enrichment and inherited s-process enrichment from the host galaxy as plausible explanations for the observed overabundances. Our chemically peculiar subset of intrinsic carbon and s-process enriched binary post-AGBs also hints at potential variation in the efficiency of chemical depletion between stars with C-rich and O-rich circumbinary disc chemistries. However, critical observational studies of circumbinary disc chemistry are necessary to address gaps in our current understanding of disc-binary interactions inducing chemical depletion in binary post-AGB systems.

==> Null.tex <==
%Table 2

\begin{landscape}
    \begin{table}
        \caption{Photometric data of the targets. See text for full details.}
        \begin{center}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{ c c c c c c c c c c c c c c c c c c c c c }
            \hline
            Object Name & RA ($\degree$) & Dec ($\degree$) & U & B & SDSS.RP & V & R & I & J & H & K & W1 & W2 & AKARI.S9W & IRAS.F12 & W3 & W4 & IRAS.F25 & IRAS.F60 & IRAS.F100\\
            \hline
            J005107  & 12.780083 & -73.692598 & 16.65 & 16.657 & 99.99 & 15.84 & 15.45 & 14.85 & 14.33 & 13.65 & 12.93 & 11.39 & 10.44 & 99.99 & 99.99 & 8.365 & 6.926 & 99.99 & 99.99 & 99.99 \\
            MACHO 47.2496.8  & 73.930267 & -67.852718 & 17.31 & 16.23 & 99.99 & 15.08 & 14.28 & 14.00 & 13.19 & 12.67 & 12.57 & 12.09 & 11.79 & 99.99 & 99.99 & 10.26 & 9.248 & 99.99 & 99.99 & 99.99 \\
            HD 158616 & 262.695520 & -11.368968 & 11.92 & 10.09 & 9.368 & 9.642 & 99.99 & 99.99 & 7.845 & 7.299 & 6.525 & 5.178 & 4.029 & 3.301 & 3.520 & 2.600 & 1.234 & 2.900 & 1.600 & 1.980 \\
            V453 Oph  & 261.704705 & -2.393453 & 12.29 & 11.90 & 10.30 & 10.85 & 10.50 & 9.791 & 8.806 & 8.442 & 8.283 & 7.993 & 7.890 & 99.99 & 99.99 & 7.743 & 7.549 & 99.99 & 99.99 & 99.99 \\
            \hline
            \end{tabular}
            }
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The RA and DEC coordinates are given for the J2000 epoch. Null magnitudes are listed as 99.999.
        \end{tablenotes}
       
        \label{tab:photometry}
    \end{table}    ,
\end{landscape}




%Table 1

\begin{landscape}
    \begin{table}
        \caption{This table lists the object name and alternative widely used name for each object in the sample along with two sets of stellar parameters. The final column lists the references to the literature analysis.}
        \begin{center}
            \begin{tabular}{ c l l c c c c c c c c c c  }
                \hline
            \#ID & Object Name & Other Name & \begin{tabular}[c]{@{}l@{}}\Teff\\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & & \begin{tabular}[c]{@{}l@{}}\Teff \\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & Ref. \\
                \hline
        		\multicolumn{3}{ c }{} & \multicolumn{4}{c }{This Study} & \multicolumn{5}{c }{Literature} \\
                \hline
                1 & J005107.19-734133.3 &	OGLE SMC-T2CEP-18	& 5768 $\pm$ 100	&	0.21 $\pm$ 0.10	&	-1.57 $\pm$ 0.10   &	4.08 $\pm$ 0.50	& & 5267 $\pm$ 250	&	0.72 $\pm$ 0.50	&	-1.56 $\pm$ 0.50  & ... & 1	\\
                2 & MACHO 47.2496.8 &	OGLE LMC-T2CEP-15	&
                4898 $\pm$ 100	&	0.00 $\pm$ 0.50	&	-1.42 $\pm$ 0.16   &	4.00 $\pm$ 1.00	& & 4900 $\pm$ 250	&	0.00 $\pm$ 0.50	&	-1.50 $\pm$ 0.50   &	3.50 $\pm$ 1.00  &	2\\
                3 & HD 158616 &	IRAS 17279-1119	& 7379 $\pm$ 110	&	1.47 $\pm$ 0.25	&	-0.50 $\pm$ 0.20   &	2.97 $\pm$ 0.25 &  & 7250 $\pm$ 125	&	1.25 $\pm$ 0.25	&	-0.64 $\pm$ 0.12 &	3.00 $\pm$ 0.50 &	3\\
                4 & V453 Oph &	BD-02 4345	& 	6158 $\pm$ 100	&	1.19 $\pm$ 0.25	&	-2.27 $\pm$ 0.10   &	2.50 $\pm$ 0.50 &  & 6250 $\pm$ 250	&	1.50 $\pm$ 0.50	&	-2.23 $\pm$ 0.12   &	3.00 $\pm$ 0.50 & 4\\
                \hline
            \end{tabular}
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The stellar parameters under "This study" represent the spectroscopically determined atmospheric parameters obtained using the $Python$ wrapper of i-Spec whereas the stellar parameters under the title "Literature" represent the spectroscopically determined atmospheric parameters from the Literature analysis. Note that the low-resolution spectral analysis of J005107.19-734133.3 did not provide an estimated \mv value. Detailed information on the tabulated information can be found in the individual studies identified in column 'Ref'. The column 'Ref.' indicates the individual study: 1 - \cite{Kamath2014}, 2 - \cite{Reyniers2007}, 3 - \cite{desmedt2016}, 4 - \cite{Deero2005}\\
        \end{tablenotes}
       
        \label{tab:sample}
    \end{table}    ,
\end{landscape}


==> scratch <==



The SPHERE/IRDIS polarimetric images provide a unique opportunity to directly measure the scale height of the disc for systems wi


where the mid-plane of the disc can be traced. We note that the disc mid-plane refers to the equatorial plane of a circumbinary disc, which is where most of the dust and gas are concentrated. The mid-plane appears as a dark region that separates resolved scattered light emission from upper and lower surfaces of highly inclined disks ($i>40^{\circ}$). }


The reduced images from our observations of AR Pup and the reference stars are shown in Figures 2 and 3 for ZIMPOL and IRDIS, respectively. The stacked ZIMPOL images in both
filters show a bright core that is elongated in the northeast to southwest direction. The same elongation can be surmised in the IRDIS data. Deconvolution of the ZIMPOL images reveals
a clear “double-bowl” structure separated by a dark layer band. This is similar to the appearance of edge-on protoplanetary disks. We thus interpret the dark layer band as the optically thick disk mid-plane and the two “bowls” as the two disk surfaces scattering the starlight. We see no indication of direct stellar light reaching us through the disk, while the higher resolution images in Vand Iband provide stronger constraints than the Hband image. In the Vand Ibands we see no indication of direct stellar light reaching us through the disk (no central point source is visible).

\textbf{For systems with a visible mid-plane, we
